HoloSpot: Intuitive Object Manipulation via Mixed Reality Drag-and-Drop

Human-robot interaction through mixed reality (MR) technologies enables novel, intuitive interfaces to control robots in remote operations. Such interfaces facilitate operations in hazardous environments, where human presence is risky, yet human oversight remains crucial. Potential environments include disaster response scenarios and areas with high radiation or toxic chemicals. In this paper we present an interface system projecting a 3D representation of a scanned room as a scaled-down 'dollhouse' hologram, allowing users to select and manipulate objects using a straightforward drag-and-drop interface. We then translate these drag-and-drop user commands into real-time robot actions based on the recent Spot-Compose framework. The Unity-based application provides an interactive tutorial and a user-friendly experience, ensuring ease of use. Through comprehensive end-to-end testing, we validate the system's capability in executing pick-and-place tasks and a complementary user study affirms the interface's intuitive controls. Our findings highlight the advantages of this interface in improving user experience and operational efficiency. This work lays the groundwork for a robust framework that advances the potential for seamless human-robot collaboration in diverse applications. Paper website: https://holospot.github.io/

==> sections/apendix.tex <==
\section*{APPENDIX}

==> sections/related_works_old.tex <==
\vspace{-0.1cm}

\section{\textbf{RELATED WORKS}}
The intersection of Mixed Reality and Human-Robot Interaction has become a dynamic research area, with numerous studies exploring the potential of MR to enhance robotic control and human collaboration in complex environments. We highlight a selection of recent and particularly pertinent studies.

\subsection{\textbf{Control via Mixed Reality Interfaces}}

Recent advancements in MR technologies have significantly impacted HRI, particularly in scenarios requiring intuitive control and enhanced situational awareness.
Previous studies have demonstrated the effectiveness of MR interfaces in improving operator control over robotic systems, particularly in environments where traditional 2D interfaces fall short. 

For example,~\cite{chen20233d} developed a VR-based interface that enables real-time visualization and manipulation of robotic systems. Their work demonstrated the advantages of using 3D interfaces to overcome the limitations inherent in 2D displays, allowing operators to control robots with greater precision and efficiency.

Additionally, the study by \cite{iglesius2024mrnab} explores the fusion of MR with robotic systems, particularly focusing on the application of MR in scenarios requiring intricate spatial understanding and collaboration. Their research highlights the use of MR to facilitate HRI in environments that are traditionally challenging for robot navigation and manipulation, underscoring the potential of MR technologies in HRI.

\subsection{\textbf{3D Instance Segmentation and Grasp Pose Estimation}}

Understanding and interacting with complex environments is a fundamental challenge in robotics, which is often addressed through 3D instance segmentation and grasp pose estimation. The Spot-Compose framework, introduced by \cite{lemke2024spotcompose}, is an advanced approach to these tasks. This framework utilizes a combination of sophisticated algorithms to segment 3D scenes and localize objects, making it particularly effective for tasks like object retrieval and manipulation. 

Building on the concepts of 3D instance segmentation, the OpenMask3D framework \cite{takmaz2023openmask3d} offers a powerful tool for segmenting and identifying objects within complex scenes. OpenMask3D employs visual-language models (VLMs) to perform open-vocabulary segmentation, allowing segmentation and identification of arbitrary objects within a scene, enhancing the robot's ability to interact with diverse and previously unseen items based on natural language descriptions. This capability is critical in environments where the robot must adapt to new and unseen objects, enhancing its operational flexibility and effectiveness.

In parallel, grasp pose estimation has seen substantial progress through the development of AnyGrasp, a framework introduced by \cite{fang2023anygrasp}. AnyGrasp predicts two-finger grasps directly from 3D point clouds, using a dense supervision strategy that incorporates real perception data and analytic labels. This method accounts for factors such as the object's center-of-mass and environmental constraints, ensuring stable and collision-free grasps. 

By combining these advanced segmentation and grasping techniques, robots are equipped with the necessary tools to perform dynamic and precise manipulation tasks in varied and unpredictable settings.

\subsection{\textbf{Human-Robot Collaboration in Hazardous Environments}}

The deployment of robotic systems in hazardous environments is critical for minimizing human exposure to dangerous conditions while maintaining essential oversight. In such settings, human-robot collaboration becomes indispensable. Research has increasingly focused on developing interfaces that enhance this collaboration, particularly in environments where traditional methods of operation are challenged by factors such as restricted visibility, heightened risks, or the necessity for accurate, real-time decision-making.

\begin{figure*}[t]
\vspace{-0.5cm}
\centering
\includegraphics[width=\linewidth]{ root_images/paper_pipelines_1.png}
\caption{\textbf{System overview.} 
Our method relies on both offline and online segments. Offline segment (left), is used to construct 3D scene that will be utilised in the subsequent online phase. The online segment (right) is used to control the Boston Dynamics Spot \cite{spot} using the Microsoft HoloLens 2 \cite{hololens} with the help of an online server.}
\label{fig:system_overview}
\vspace{-0.5cm}
\end{figure*}

A notable example is the work by CERN ATS on developing an MR interface for remote operations in accelerator facilities \cite{CERN2023}. This system was designed to allow operators to control robots within hazardous accelerator environments, where human presence is restricted due to safety concerns. By integrating MR, the interface enables users to interact with a virtual representation of the environment, enhancing their ability to perform complex tasks with greater precision and situational awareness.

Complementing this, \cite{lunghi2019multimodal} investigated the use of MR for robotic operations in environments contaminated with toxic chemicals. The study demonstrated that MR could significantly improve the operator’s ability to navigate and manipulate objects in these environments, thus reducing the risk to human life and enhancing the efficiency of robotic interventions.
